SonifyAR: Context-Aware Sound Generation in Augmented Reality

Sound plays a crucial role in enhancing user experience and immersiveness in Augmented Reality (AR). However, current platforms lack support for AR sound authoring due to limited interaction types, challenges in collecting and specifying context information, and difficulty in acquiring matching sound assets. We present SonifyAR, an LLM-based AR sound authoring system that generates context-aware sound effects for AR experiences. SonifyAR expands the current design space of AR sound and implements a Programming by Demonstration (PbD) pipeline to automatically collect contextual information of AR events, including virtual content semantics and real world context. This context information is then processed by a large language model to acquire sound effects with Recommendation, Retrieval, Generation, and Transfer methods. To evaluate the usability and performance of our system, we conducted a user study with eight participants and created five example applications, including an AR-based science experiment, an improving case for AR headset safety, and an assisting example for low vision AR users.

==> Sections/Archive/1-Introduction-old.tex <==
%%
\section{Introduction}
%In recent years, Augmented Reality (AR) has evolved into an interdisciplinary domain, offering users multi-modal information to enhance immersive experiences. Beyond the visual component, auditory feedback has been demonstrated to play a pivotal role in heightening immersion [CITE]. 

%Sound, as a effective addition to human-computer interfaces \cite{zhou_role_2007}, has been proved powerful in improving Augmented Reality (AR) experiences [cites]. 
The role of sound in Augmented Reality (AR) has grown profoundly, becoming a pivotal element that adds depth and immersion to user experiences, such as depth perception and task completion \cite{zhou_role_2007}, search and navigation \cite{ruminski2015experimental} and even assistance for visually impaired people ~\cite{ribeiro_auditory_2012}. Despite the potential of sound in AR, its integration—particularly in the scope of sound authoring—remains inadequately addressed. Current AR authoring platforms like \textit{Reality Composer} \cite{realitycomposer}, \textit{Adobe Aero} \cite{adobeaero}, and \textit{Unity} \cite{unity-website} provide only rudimentary sound authoring support. Central to these platforms is the \textit{Programming by Specification} (PbS) methodology \cite{monteiro2023teachable}, where designers define AR sound content and play conditions during the design phase, which is also addressed as the ``\textit{trigger-action mechanism}'' \cite{monteiro2023teachable}. A ``\textit{trigger}'', such as tapping an AR object or a specific location in the scene, sets the condition for launching certain actions. Subsequently, an ``action'', whether it be the playing of an animation or a sound effect, responds to the earlier trigger. This allows creators to precisely define the conditions for triggers and the consequent sound effects. Although widely explored, these current authoring workflow present three critical gaps in terms of AR sound authoring:

% These tools, which mostly involves Programming by Specification (PbS), require user to specify AR sound content in the design phase. For example, one of the most commonly adopted authoring method is trigger-action mechanism, where a "trigger" (e.g., tapping an AR object, or user getting close to a certain position) is an event or condition for initiating specific actions, and an "action" (e.g., playing animation or sound effect) is the triggered response. Creator needs to explicitly specify the trigger conditions and the corresponding sound effects. These existing AR authoring capabilities has three major deficits:

\begin{enumerate}
    \item \textbf{Limited sound interaction space.} Since action triggers are typically bound to virtual objects, sound effects for interactions between AR objects and the real-world environment (\textit{e.g.}, a virtual ceramic cup clinking against a wooden table) or between the user and the real-world via the AR interface (e.g., a user tapping on a wall through AR interface) are neglected.

    \item \textbf{Lacking real-world context.}  As authoring happens before AR experiences, key context information can be missing for creating matching sound effects. For instance, authoring the sound of a virtual ball dropping on real world surfaces is challenging since there is no contextual information regarding the surface material.
    
    \item \textbf{Limited sound source.} Given the limited availability of sound assets in the default library that comes with authoring platform and the scarcity of suitable sound resources online, AR authors struggle to find fitting sounds for distinct AR events. Examples include reproducing the the wing flutter sound of a virtual dragonfly or simulating footsteps of a virtual robot traversing diverse surfaces like wood, carpet, or glass. 
\end{enumerate}

%However, sound authoring in AR has been an under-addressed topic. Existing AR authoring platforms, such as Reality Composer \cite{realitycomposer} and Adobe Aero \cite{adobeaero}, offer only basic support for sound authoring. The sound authoring capabilities in these tools primarily use trigger-action mechanisms—where a "trigger" (e.g., tapping an AR object, or user getting close to a certain position) is an event or condition for initiating specific actions, and an "action" (e.g., playing animation or sound effect) is the triggered response. Such a sound authoring approach is limited in several aspects:

%\begin{enumerate}
    %\item It offers a limited range of AR interactions. Since the AR system only possess information about the virtual object in the authoring stage, the potential sound interaction is limited to the virtual object itself. Thus it fails to cater to sound effects that depict interactions between AR objects and the real-world environment (\textit{e.g.} a virtual ceramic cup coming in contact with a wooden table) and also between user and the real world environment through AR interface (\textit{e.g.} user tapping on wall in AR). 
    
    %\item Because the authoring process occurs before the actual AR experience, it is not possible to adapt the authored sound to real-time context factors, such as the location of virtual objects or the material of the real-world surface. Consequently, the authored AR sound lacks context awareness. %During the AR experience, if a user taps or drags an AR object, and the sound isn't predetermined during the authoring phase, it won't be played during the experience, even when specific interactions should produce sound.
    
    %\item It lacks support for finding suitable sound assets, particularly for niche AR events. Given the limited availability of sound assets in the default list provided by the software and the scarcity of suitable sound resources online, users may encounter difficulty in creating matching sounds for specific AR events, such as replicating the wing flutter sound of a virtual dragonfly or simulating footsteps of a virtual robot on various surfaces like wood, carpet, or glass.
%\end{enumerate}

To address these challenges, we present \textit{SonifyAR}: a context-aware AR sound authoring system using generative models. SonifyAR harnesses the advancements of Large Language Models (LLMs) and sound acquisition models to recommend, retrieve, and generate context-aware sound effects in response to AR events. Inspired by prior work like \textit{Rapido} \cite{leiva2021rapido}, \textit{PoseVec} \cite{zhang2023posevec} and \textit{GestureAR} \cite{wang2021gesturar}, our approach adopts a \textit{Programming by Demonstration} (PbD) \cite{10.1145/291080.291104} pipeline that enables users to discover and author context-aware AR sound during AR interaction.  Our authoring system identifies potential sound-producing AR events and utilize LLM and sound acquisition models to generate context-aware sound effects in real time. To our knowledge, we are the first system to offer automatic, in-context sound authoring for AR. 

%Our SonifyAR system fills the previously mentioned deficits. First, the PbD authoring pipeline enables inclusion of context information to the AR sound authoring, enabling us to expand the AR sound interaction space and include user-environment and virtual object-environment sound interaction. Second, 

%In order to expand the limited interaction for AR sound, we propose and demo an expanded AR sound design space that includes user-environment and virtual object-environment sound interaction.

To design SonifyAR, we discuss and justify three major design choices in Section 3. Firstly, drawing inspiration from Jain et al. \cite{jain_taxonomy_2021}, we analyze the auditory design space of AR interactions and describe the design space as a triad between user, virtuality and reality. We further choose ? prototypical AR interaction types spanning the triad for our implementation. Secondly, we explore methods for capturing and representing context information of AR interactions. Thirdly, we compare and summarize different existing sound acquisition pipelines and select recommendation, generation, and retrieval methods for implementation. We introduce the implementation of SonifyAR in Section 4 and evaluate its usability in Section 5.

%OLD VERSION, we established a design space for AR sound centered around three core elements: the user, virtuality, and reality. We cataloged potential interactions among these three entities, identified the currently supported sound interactions by the existing AR authoring tools, and proposed enhancements to include both user-environment and virtual object-environment sound interactions. Based on this extended design space, we implemented our context-aware AR sound authoring pipeline with phone-based AR, LLM and audio generative model. To validate our system's usability, we conducted a hands-on study to compare our authoring pipeline with existing tools.


%Through our evaluations, we've found that our system significantly reduces the time needed to integrate sound effects into AR and yields sound effects that are more contextually appropriate compared to traditional authoring pipelines.

% In general, our work features three main contribution in the realm of AR sound authoring. 
% 1) We enlarge the AR sound authoring design space by including AR sound events caused by user interacting with real world and virtual object interact with real world. 
% 2) We propose and implement a generative model based sound authoring pipeline that outputs sound assets using contextual information of real-time AR interaction. 
% 3) We explore a novel event-based AR authoring method and demonstrate its advantage over  existing method by interviewing AR experts. 

The contributions of this paper are summarized as follows:
First, we explored the landscape of sound authoring in AR, identifying a noticeable gap between the existing authoring tools and the broader potential opportunities in the design space. Second, to address this gap, we introduce an AR sound authoring pipeline that incorporate context information of the environment, virtual object, and user action. Lastly, we implement this proposed pipeline as an LLM and generative model based sound authoring system. This implementation is evaluated with eight participants for usability and future application opportunities.  

Our work makes three primary contributions: (1) a design space for AR sound authoring tools, which highlights existing gaps in the literature; (2) a novel context-aware AR sound authoring pipeline using generative AI, called SonifyAR, that incorporates sensed environmental cues, virtual object, and user action; (3) findings from a user study with eight designers and five application examples that demonstrate SonifyAR's potential and key advancements in this space.

==> Sections/Archive/2-Related_Works.tex <==
\section{Related Work}
%[Could be a short related work section as we are aiming for a short paper]
\subsection{AR Sound Authoring}
%Main point here is, AR sound is proved powerful by many prior work, but it's under addressed in current literature and frameworks.
Prior investigations demonstrate that sound is crucial in AR experiences by directing the user's attention, enhancing the sense of presence, and creating interactive time-varying experiences \cite{serafin_sonic_2018}. Nonetheless, the current landscape of AR authoring tools and platforms reveals a deficiency in adequately supporting AR sound authorship.
These AR authoring tools exhibit a spectrum of fidelity and application scenarios \cite{monteiro2023teachable,nebeling_trouble_2018}. Tools with lower fidelity, like Halo AR \cite{haloar} and ARVid \cite{arvid}, empower users to overlay virtual imagery, videos, and 3D assets onto the real world. In these tools, sound elements are typically integrated directly into virtual assets (e.g. videos with sound or virtual animals that roar). Moving up the fidelity scale, tools like Adobe Aero \cite{adobeaero} and Apple's Reality Composer \cite{realitycomposer} provide trigger-action interactions. Here, sound elements can be selected and edited through user-friendly interfaces and linked to triggers like user taps or proximity events. High-fidelity tools, such as Unity \cite{unity-website} and Unreal \cite{unreal-engine-website}, offer both visual editors and coding capabilities. They provide substantial flexibility in designing AR sound interactions, including the ability to set parameters like sound decay and code-specific conditions for activating sound assets.


While most AR authoring tools support sound editing, significant gaps remain in their AR sound authoring capabilities. As previously noted, creators are often tasked with sourcing suitable sound effects to match specific sound-producing events. Additionally, the range of events that can be associated with sounds is limited. Our proposed system aims to address these issues.

% Although AR sound are supported by almost all AR authoring tools, we still see major deficits in their AR sound authoring capabilities. For one, there are little or no support for sound asset creation. Creator needs to browse or record their own sound assets, posing substantial obstacle for amateur creators to author immersive AR sound; 
% For two, sound experiences are created before actual AR experiences, thus lacking contextual information and compromising overall immersive quality.
% We aim to fill these gap by implementing a PbD interface that generates sound assets for AR experiences in real-time.
%High fidelity tool (Unity, Unreal), mid-fidelity tool (Aero, Reality Composer) ,low fidelity tool (), mid-fidelity tool. Trigger-action. Code based. Many settings and rendering options, but no support for sound generation, especially having context involved.

\subsection{Context-awareness in AR}
%The target is to show how existing work address context awareness, while neglecting the sound modality
%[Emphasize there's no dedicated tool for sound authoring in AR]
Context-aware applications adjust their functionalities to align with the current context, enhancing usability and tailoring experiences for different operating conditions~\cite{abowd1999towards}.
In AR, context-awareness ensures that the application adapts not only to the user but also to their environment and specific needs, making the application more user-friendly and immersive \cite{krings_development_2020}. There have been many prior work addressing the context-awareness in AR, focusing on context information like location, scene semantics and human factors. Popular AR game PokemonGo, for example, shows game contents based on user's physical location. A more common practice in AR research is adapting virtual contents to scene semantics---essentially understanding the objects and their locations in the user's environment. Qian et al. \cite{qian2022scalar} introduced an authoring system that helps user create adaptive AR experiences to surrounding scene semantics. Lang et al. \cite{lang2019virtual} analyzes scene semantics to guide the positioning of virtual agents. Similarly, Liang et al.~\cite{liang2021scene} places virtual pets into AR based on scene geometry and semantics. This realm of similar work \cite{han2020live,tahara_retargetable_2020} usually captures and analyzes surrounding environment, and designs algorithms that determines possible interaction between virtual content and real-world scene.  Lindbauer et al. \cite{lindlbauer2019context} push the AR context-awareness further by including task and cognitive load as context to adjust level of detail of AR virtual interface.
Although there has been substantial discussion in the realm of AR context-awareness, we observed that prior work generally focuses on the visual modality of AR, neglecting sound. Additionally, existing work primarily concentrates on adjusting and arranging virtual content rather than generating new content. We aim to fill this gap by designing a sound generation pipeline that processes context information to produce matching sound assets.


\subsection{Sound Acquisition}
%Show existing methods in sound synthesis, which works as basis of our work.
Many methods can be used to retrieve, synthesize or generate sound for AR experiences. For example, Oncescu et al.~\cite{Oncescu21a} trained cross-modal embedding models to support text-to-audio retrieval. Multi-modality models like VAST ~\cite{chen2023vast} also supports text-to-audio retrieval that could potentially be used to provide sound assets for AR experiences. Similarly, FreeSound \cite{freesound} implemented an online API that retrieves sound effects from dataset of professional assets with text. Besides retrieval methods, text-to-audio generation models \cite{liu2023audioldm,yang2023diffsound,kreuk_audiogen_2023} also emerge with promising performance and could be used to acquire sound for niche cases of text description. In general, retrieval methods can provide more realistic sound assets but do not ensure coverage for all text descriptions. While generative models might not achieve same sound quality, they can produce results for any text input. In SonifyAR, we adopt both the retrieval method and the text-to-audio generation model to utilize their complementary strength. Specifically, we use the FreeSound API for its extensive library of professional sound asset and AudioLDM~\cite{liu2023audioldm} for its state-of-the-art performance on sound generation. 


Besides retrieval and generative models, sound synthesis with physics\cite{raghuvanshi_interactive_2006,roodaki_sonifeye_2017,ren_example-guided_2013,jin_deep-modal_2020,jin_neuralsound_2022,liu_sound_2021,diaz_rigid-body_2022} are also widely explored to acquire sound assets. Traditionally using methods like spring-mass model \cite{raghuvanshi_interactive_2006} and recently improved with deep learning \cite{jin_deep-modal_2020}, these synthesis methods can provide realistic sound simulation given 3D model and material properties. However, we did not pursue this line of work due to the challenges associated with providing precise 3D models of environments and the computational cost.

==> Sections/Archive/3-Design_Space.tex <==
\section{The Auditory Design Space of AR}
\label{section:design space}
% \section{The Soundscape of AR}
% See https://dl.acm.org/doi/abs/10.1145/3461778.3462106 for some hints.
Sound in AR stands as a pivotal modality, not merely as an ambient element but as an interactive feature that can be integrated at various stages, events, or interactions. Inspired by Jain et al.~\cite{jain_taxonomy_2021} on VR sound taxonomy , we aim to enumerate the sound interaction possibilities in AR by classifying the sounds. While Jain et al. categorize VR sound by source and intent, our emphasis is on the parties involved in audible interactions. We conduct a comprehensive analysis of the broader design space for AR sound interaction, focusing on the three key components of AR: user, virtuality and reality. By identifying opportunities that have not been well addressed by existing tools, we propose solutions to expand the interactive auditory space in AR.
%expand the table and see if it's a better way to present


\paragraph{The Triad of User, Virtuality, and Reality}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/Design Space.pdf}
    \caption{The sound-producing opportunities in the triad of User, Virtuality and Reality. Dashed boxes indicates the supported sound interaction space by existing tools and the expanded interaction space envisioned by our work. AR events shown in red text are examples.}
    \label{fig:triad}
\end{figure}


In a typical AR interaction, there are three main components involved: \textbf{the user}, representing the individual experiencing or interacting with the AR; \textbf{virtuality}, referring to the virtual object(s) placed in the AR experience; and \textbf{reality}, denoting the physical environment in the real world that hosts the AR experience.

Based on this triad, we list potential sound-producing interactions in an AR session, which could involve one or more components (see \figref{triad}). Note that while some parties naturally produce sound (e.g., users can generate sounds either through their own actions or by directly interacting with the physical world), our interest lies in events where the AR system (\textit{e.g.} smartphone or AR glasses) generates the sound. Thus, sounds naturally generated by user and reality are excluded in our discussion.

\begin{itemize}
    \item \textbf{Virtuality:} Sounds can generate from the internal activities of a virtual object. This could be bound to an object appearing or disappearing (\textit{e.g.} a notifying sound when a virtual object show up), or from an object's animated behavior (\textit{e.g.} the mechanical noise made by a moving robot or a virtual dinosaur roars). Also, multiple virtual objects can also interact in a manner that produces sound. For instance, a virtual ball might produce a sound when hitting a virtual wall. These sound aspects are well supported by existing tools like Reality Composer and Adobe Aero.
    \item \textbf{User-Virtuality:} When a user interacts with a virtual object, for instance tapping on a virtual dog, a corresponding sound, such as a bark, could be generated as feedback. In most AR creation tools, the trigger and its corresponding sound feedback can be predefined by specification in the authoring phase. In general, this sound aspect has also been well supported by existing tools.
    \item \textbf{User-Reality:} This type of event refers to users interact with the physical environment via their AR devices, even when no AR objects are present. A specific example would be a user tapping on a real-world surface through their AR device (\textit{e.g.} tapping on a wooden surface in phone screen). Sound feedback can enhance these interactions. From an accessibility perspective, such auditory cues can assist individuals with low vision, aiding them in understanding the material properties of their surroundings through AR. This sound feedback can also benefit overall immersiveness of the AR experiences, and potentially improve task performance. However, we have noticed a lack of support for this interaction type in mainstream authoring tools.
    \item \textbf{Virtuality-Reality:} This landscape highlights a significant gap that many existing AR authoring systems overlook: the interaction between virtual and real objects. For example, when a virtual metallic robot walks on an actual glass table,  a stomping sound, resulting from the collision between metal and glass, should be produced. However, no existing AR authoring tools offer straightforward implementation for such AR sound. 
    \item \textbf{User-Virtuality-Reality:} When a user-initiated action involves both virtual object and the real world environment, sound can be provided as feedback to validate this action and improve immersiveness. For example, user can drag and slide a virtual cup on a table surface. This action can be complemented with a material-aware sliding sound. However, due to the complexity of contextual information, we are unaware of any existing AR authoring tools that support such auditory feedback. 
\end{itemize}

Based on the above analysis and as illustrated in \figref{triad}, existing AR authoring tools, such as Reality Composer~\cite{realitycomposer} and Adobe Aero~\cite{adobeaero}, offer robust support for sound feedback in the domain of virtuality and user-virtuality interactions. However, the dimensions of virtuality-reality and user-reality are just as vital, if not more so, since they extend immersiveness beyond a purely digital domain. Yet, efficient methods for authoring sound feedback in these dimensions are conspicuously absent. While one might consider utilizing existing technologies like scene recognition and physical simulation to enhance support for user/virtuality-reality interactions, integrating these into current frameworks is not straightforward and might demand programming expertise. Therefore, developing an authoring interface that holistically supports all interaction types listed in \autoref{fig:triad} remains a significant challenge.
\begin{comment}
Specifically, we see three major challenges in authoring these unsupported sounds:
\begin{itemize}
    \item \textbf{Complexity of context information.} For sound interaction that involves more than one interaction components, the context information can include multiple sources and be in multiple forms, thus hard to collect and analyze.
    \item \textbf{Difficulty in acquiring matching sound.} For niche sound feedback like material-aware knocking sound, acquiring such sound asset can be challenging for creator. 
    \item \textbf{Difficulty in specifying trigger.} As sound feedback can be embedded in very complex context and involve multiple conditions, specifying such trigger can be challenging with either user interface or code. 
    
\end{itemize}
\end{comment}
In the subsequent section, we will discuss how SonifyAR is designed to tackle these challenges, encapsulate all listed sound interactions within one single framework, and streamline AR sound authoring with LLM and generative models.

\begin{comment}
%\cmt{maybe use a table to summarize}


\begin{tabular}{ |p{4cm}||p{4cm}|p{4cm}|  }
 \hline
 \multicolumn{3}{|c|}{Taxonomy of Interaction Sound Authoring} \\
 \hline
 Screen & User (e.g. tapping) &Virtual Content (e.g. coliding) \\
 \hline
 Virtual Content   & \checkmark    & \checkmark    \\
 Real-World Content &   X  & X  \\

 \hline
\end{tabular}

\begin{itemize}
    \item \textbf{User:} Any sound produced by the user can be classified under this category, such as the user's voice command. However, this does not fall within the scope of sound authoring in AR.


    \item \textbf{Virtuality:}
    \begin{itemize}
        \item \textbf{Virtual Object Interactions:} Much like in video games, two virtual objects can interact in a manner that produces sound. For instance, a virtual ball might produce a sound when hitting a virtual basket.
        \item \textbf{Virtual Object Internal Sound:} Sounds can generated from the internal activities of a virtual object. This could be due to an object appearing or disappearing, or from an object's animated behavior, such as the mechanical noise made by a moving robot.
    \end{itemize}


\item \textbf{Reality:}
Sounds that naturally occur in the physical environment lies in this category, such as cars passing by, the hum of an air conditioner, or a dropped glass hitting the floor. Since these sounds are purely produced by real objects, they do not fall within the scope of authored sound in AR.


    \item \textbf{User-Virtuality:} This category also refers to interactive sound feedback, which is the primary target of trigger-action-based authoring systems. When a user interacts with a virtual object, for instance by tapping on a virtual dog, a corresponding sound, such as a bark, is generated as feedback. In most AR creation tools, the trigger event and its corresponding sound feedback must be predefined.
    
    \item \textbf{User-Reality:}
    \begin{itemize}
    \item \textbf{Physical Contact Between User and Environment:} Examples include knocking on a wooden table with one's hand or opening a physical door. These do not involve the AR system.
    \item \textbf{Interaction Through the AR Lens:} This category includes instances where users interact with the physical environment via their AR devices, even when no AR objects are present. A specific example would be a user tapping on their AR device while it displays a wooden surface in the AR camera view. From an accessibility standpoint, this approach can benefit individuals with low vision, aiding them in understanding the material properties of their environment through AR.

    \end{itemize}
    \item \textbf{Virtuality-Reality:} This landscape highlights a significant gap that many existing AR authoring systems overlook: the interaction between virtual and real objects. Picture a virtual metallic robot walking on an actual glass table; there should be a distinct sound to accompany this interaction. Similarly, dragging a virtual ceramic bowl across a wooden table would require the playback of a friction-related sound.
\end{itemize}

Based on the above analysis and \figref{triad}, existing AR authoring tools, such as Aero, offer robust support for sound feedback in the domain of virtuality and user-virtuality interactions. However, the dimensions of virtuality-reality and user-reality are equally, if not more, vital, as they offer immersiveness beyond the purely digital domain. Despite their importance, they currently lack efficient methods for authoring sound feedback. While one might consider utilizing existing technologies like scene recognition and physical simulation to enhance support for user/virtuality to reality interactions, these cannot be easily integrated into the trigger-action-based framework. Therefore, developing an authoring interface that holistically supports all four interaction types remains a significant challenge.

In the subsequent section, we will discuss how \Name{} is designed to encapsulate all these types within a single framework, streamlining sound authoring in AR experience.

\end{comment}

==> Sections/Archive/4-Pipeline_of_MR_Sound_Context_Awareness.tex <==

\begin{comment}
\section{\Name{}: A Event-based Sound Authoring System for AR}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/pipeline_temp.png}
    \caption{Pipeline of \Name{}}
    \label{fig:pipeline}
\end{figure}

Our system adopts an event-based sound authoring framework. We interpret each user interaction and its subsequent result as an event. Every event is then translated into a text string and sent to LLM to determine whether a sound effect corresponds to that event. If the event is deemed sound-producing, our sound production model generates the appropriate sound effect for it. Additionally, our system maintains a list of these events, allowing users to access and manage the sound effects throughout their AR experience.

Our system consists of three primary components (See Fig X):
a) Event Detection Component: Identifies if a specific event within the AR scene should generate sound.
b) Sound Production Component: Produces sound effects for events identified as needing sound.
c) User Interface Component: Enables users to experience the AR scene and provides the capability to view, edit, and modify sound effects for all events.

Since our system is specifically designed for sound authoring in AR, it does not provide the capability to directly create or modify the overall AR scene. Instead, it accepts AR scenes created by other tools as input. Given its focus on sound, our system can either function as a plug-in for existing AR authoring tools, enhancing the sound authoring functionality, or it can operate as a standalone AR experience loader, giving users the experience of an AR scene with real-time sound feedback.

In the subsequent sections, we start with a brief overview of the file format for pre-designed AR scenes. Following that, we delve into the workflow of each of the system's main components. Finally, we detail the system's implementation specifics.

\subsection{Background of AR Scene Structure}
Our system is designed to process pre-crafted AR scenes as input. Thus, a brief overview of AR scene components is essential. There are various AR authoring systems exist, ranging from simpler ones like Reality Composer to more professional-facing platforms like Unity. To ensure our framework's versatility across most AR scenes, we use AR scenes created by Reality Composer as our input. This choice is due to its lightweight nature and its provision of essential information needed for our system's sound authoring. We employ this approach as a proof-of-concept. 
While AR scenes from different tools might have slight structural or naming variations, they should be convertible to the similar format. Therefore, as long as other tools provide the required information, they can integrate with our framework.

A standard AR scene comprises \textit{AR objects} and \textit{behaviors}. AR objects refer to 3D models, either static or animated, arranged in a user-defined layout. Every AR object possesses a filename that may indicate its nature or identity. If needed, a more detailed description can be embedded within the 3D model's metadata. Behaviors typically combine a trigger with an action. Triggers can be user interactions, such as tapping an AR object, the camera approaching an AR object, or a programmable event. In contrast, actions denote intended outcomes, like initiating an animation, causing an AR object to appear/disappear, or altering an AR object's position or orientation. In trigger-action-based AR authoring systems, users can associate triggers with actions, orchestrating the sequence of events in the AR scene. Many AR authoring tools, including Reality Composer, Adobe Aero, and Unity, offer trigger-action specification.



% Our system accepts pre-crafted AR scene as input. Thus, it is necessary to briefly introduce the basic components of an AR scene. 
% There exists many type of AR authoring system
% from some easy system like Reality Composer to more professional system like Unity. To make sure our system framework is generic enough to support most of the AR scene, we choose to use AR scene created by Reality Composer as input, as it is lightweight and contains the minimal set of information required for sound authoring by our system.
% We use this implementation as a proof-of-concept to illustrate our framework and other more complex tools be naturally adapted to the same framework. using the same framework as long as they have the necessary information required by our framework




\subsection{Event Detection Component}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/event_temp.png}
%     \caption{Event recognition.}
%     \label{fig:event}
% \end{figure}

 

In trigger-action-based AR authoring system, creators predetermine which events can produce sound effects. These decisions are made during the authoring phase. As a result, users can only hear sounds tied to these specific events during demonstration phase. Additionally, creators must source the right sound effects either by searching online or recording them independently.

To simplify the creation of sound effects in AR, we introduce an event-based framework. In our system, an "event" starts with a user's action, such as tapping an object (real or virtual) or dragging a virtual item, and concludes with a corresponding response, like playing an animation or ending the drag action. During such event, our system identifies both the entities involved (whether real or virtual) and the actions taken. This collected data is then compiled into a text prompt template, which is subsequently sent to the sound production component to craft the corresponding sound effect.



\paragraph{Scene Recognition}
Before generating text descriptions of events, our event detection component analyzes the physical environment captured by the camera. We use a computer vision model ([CITE]) to semantically segment the scene, identifying the material of each section.  This information is crucial for producing appropriate sound effects when either the AR object or the user interacts with real-world components (See Fig X).

\paragraph{Event-to-text}
As highlighted earlier, every event is identified and then translated into a text description which encapsulates the associated entities and actions.
To structure these descriptions, we employ a text template. This template is designed as follows: "[User action] performed on [Source Object] triggered [Behavior] on [Target Object], supplemented by [Additional Information on Involved Entities]".

Breaking this down, here are the five core components of the template:

1) User's Action: This pertains to gestures the user engages in, such as tapping, dragging, and other recognizable actions.
2) Source Object: This is the object directly acted upon by the user or the one triggering a predefined event. It can be either virtual or real entities.
3) Triggered Behavior: This can be of two types:
Predefined Behavior: Actions predefined in the AR authoring system, such as playing animations or making objects appear/disappear.
Detected Behavior: Interaction between two objects, like a user dragging an object into collision with either a physical or virtual entity. This is determined through collision detection executed on the target object.
4) Target Object: This is the object which the source object interacts with or affects. It can be either virtual or real entities.
5) Additional Information: Details that further elucidate the source object, the triggered event, and the target object. Examples encompass material descriptions of both the source and target objects and any animation details. Users are asked to provide this data within the metadata of each 3D model.

During user interaction, the system actively monitors and logs the user's interactions with objects. When an action is detected, the system retrieve the predefined behaviors and checks for other collision behaviors. The relevant information about the Source Object, Triggered Behavior, and Target Object is fetched, including any supplementary details provided in the 3D model's metadata. All this data is then plugged into the text template, crafting a coherent description that reflects the user's interaction within the AR environment. Once the text is constructed, we input it into the LLM to determine if the event produces sound. If the LLM confirms with a "yes", the event is flagged as sound-producing and forwarded to the sound production component. The resulting sound effect is then assigned to that event, ensuring it plays each time the event occurs during the AR session.
Fig X shows several sample output of user's interaction event constructed by our algorithm and its corresponding LLM response. 


% \paragraph{Pre-defined Event}
% As the AR scene begins to load, our system starts scanning the memory to identify which AR models have been loaded and what types of events have been designated for each AR object (e.g., appear/disappear, animation). Each event is then described as a natural language sentence using a template. \cmt{design and explain the template}. Once the template is populated with specific system components, the constructed sentence is sent to a language model to determine if the event requires sound. If a sound is necessary, we register this event in the "sound-producing event" list, and it is then queued for processing by the sound production component. Please refer to \cmt{Fig X} for an illustration.


% \paragraph{User Interaction Event}


\subsection{Sound Production Component}
In a standard AR authoring system, users usually access a provided sound library filled with various sound effects from which they can choose the appropriate one for a given event. If no suitable sound can be found in the library, users can search for sounds using keywords on a search engine. Once an ideal sound effect is found, it can be added to the sound library and linked to the event. 
Our system follows the similar authoring pipeline, but instead of manual selection, we utilize the LLM to automate parts of the process. 

Our system takes the text description of the event from the last step as input. Similar to other AR authoring tools, we provide a set of sound effects in a library, each labeled with a descriptive file name, like "button click" or "dog woof". The LLM then selects the most fitting sound effect from our library based on this description, and the selected sound effect is automatically linked to the event.

While our library is extensive, it may not always contain the desired sound effect. In such cases, we employ the FreeSound API [CITE] as a backup solution. This API returns a list of sound effects and descriptions based on a given query (which is our event description text). We then leverage the LLM to select the top five matches from the entire set of sound effects returned by the API, by comparing the text descriptions of the returned sound effects with our input text description. The LLM determines the most relevant matches based on the similarity between these descriptions. These selected top five alternatives are then stored in our system for users who wish to explore more options.

In the event that the desired sound effect is still not identified using the aforementioned methods, we naturally turn to the text-to-audio generation model (AudioLDM [CITE] in our implementation). Since our system already operates with text descriptions as input, this model serves as an intuitive choice for generating sound effects not covered by the previous approaches. The text-to-sound model uses the provided text description to generate the required sound effect. This newly generated sound are then stored in our system for user exploration at a later time. This method ensures that even if a sound is not present in our library or in the search engine results, we can still provide a suitable option by generating a new sound effect directly from the event description recorded by our system.

All sound generation and retrieval processes run in parallel on the backend, ensuring no interference with the user's AR experience. The user is notified upon completion of the sound generation process. See Fig. X for demonstration.
In the following section, we discuss how our system enables users to preview, select, and edit sound effects using our interface.



% We use three types of technique to generate sound given a text description.
% 1. retrieve on collection (LLM recommendation based on title)
% 2. retrieve on online resources (we use freesound)
% 3. text-to-sound generation (AudioLDM), explain details in implementation (if else).

\subsection{User Interface}

Our system adopts an in-context authoring framework, enabling users to interactively author sound effects while engaging with the AR environment. This approach enables a more intuitive authoring experience by helping users understand the relationship between their interactive behaviors and the potential generated sound effects.

To support this experience, our system does not distinctly separate the authoring and demonstration stages. We initiate our system with the AR experience created by a general AR authoring tool, and users can interact with the scene as they wish. Meanwhile, all previously mentioned components run concurrently in the background. When an event is detected, the sound generation component is activated, a text prompt appears, and a loading circle spins adjacent to the prompt, indicating the progress of the sound generation component. Once the sound generation for that event is complete, a check marker appears next to the text prompt.

An event list menu overlays the top of the AR scene, enabling users to browse all detected events and available sound effects for each event. Users can click on a sound effect to preview it and select it as the sound at runtime if deemed appropriate. Additionally, our system allows users to view the text description used to generate the sound. If the text description is inaccurate, users can propose a customized description and send it to any of the three approaches for re-generating the sound effect. This feature provides users with the flexibility to select sound effects based on their subjective judgment.

Figure X illustrates the core components and workflow of our interface.


\subsection{Implementation}

Describe the details of device, language (Swift?), Library (RealityKit?), semantic segmentation model, collision detection method, sound generative model...

% Implementation details on what exact model/algorithm used for each component, and our device used for testing.

% We want to emphasize that our system is focusing on sound authoring, so we need to take authored AR scene as input because creating AR scene is beyond the scope of our system. This makes our system to be use as an add-on to any other AR authoring tools like Aero. Once the AR scene is authored and launched, we initiate our system to generate sound effect to the scene.



% Some overview of the pipeline, with the diagram.
% \subsection{Context as text}
% Collect context information from multiple sources and models, turn them into text.
% \subsection{Sound from context}
% With the text containing context information, we could generate/retrieve/transfer sound to adapt to context.

% We use sound generation model, sound retrieval API, and recommendation of LLM.
% \subsection{User interaction}
% We consider user intention as part of the context information. Thus engaging user in a interaction pipeline is necessary. user could express their design intention and preferences over multiple choices in an iterative interaction based on language and UI taps.

\end{comment}

==> Sections/Archive/4-System.tex <==
\section{SonifyAR: A Context-aware Sound Authoring System for AR}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/SonifyAR Figure Pipeline V2.pdf}
    \caption{Pipeline of SonifyAR}
    \label{fig:pipeline}
\end{figure}


Drawing insights from several prior AR authoring research \cite{leiva2021rapido,zhang2023posevec}, SonifyAR adopts a Programming by Demonstration (PbD) sound authoring framework. During the authoring process, users freely interact with the AR environment. Meanwhile, SonifyAR collect interaction events that could potentially produce sound feedback, as well as their context information like detected planes and materials (\autoref{fig:pipeline} left). SonifyAR interprets each user action and its subsequent result as an AR event, \textit{e.g.,} user tap on a virtual object to trigger its animation. 
To fully encompass the context information of an AR event---which includes the state of user, the virtual object and the real-world environment---we consolidate this multi-modal information into a textual description. This text is then input into to the LLM, which serves as a controller for our three sound acquisition methods: recommendation, retrieval and generation. The LLM's response is interpreted as system actions, which are further executed by models and pipelines automatically (\autoref{fig:pipeline} middle). The sound acquisition results can be reviewed, selected and iterated by users with a call-out panel and all selected sound will be instantly applied in AR (\autoref{fig:pipeline} right). 

%Every event is then translated into a text string which include its contextual information and sent to LLM to interpret. Since sound generation can involve many different methods and AI models, we adopt LLM as a controller and universal interface to multiple sound generation methods. The reply of LLM can be then interpreted as generation actions further executed by different models and pipelines (\autoref{fig:pipeline} middle). The sound generation results can be reviewed, selected and iterated by user with a call-out panel and all selected sound will be instantly applied in AR (\autoref{fig:pipeline} right).

As illustrated in \autoref{fig:pipeline}, our system consists of three primary technical components:
a) Event Textualization: Collects context information and compile AR interaction events into text.
b) Sound Acquisition: Produces sound effects based on event context information.
c) User Interface: Allows users to experience the AR scene and provides the capability to view, modify, and test sound effects for AR events.

%Since our system is specifically designed for sound authoring in AR, it does not provide the capability to directly create or modify the overall AR scene. Instead, it accepts AR scenes created by other tools as input. Given its focus on sound, our system can either function as a plug-in for existing AR authoring tools, enhancing the sound authoring functionality, or it can operate as a standalone AR experience loader, giving users the experience of an AR scene with real-time sound feedback.

%In the subsequent sections, we start with a brief overview of the file format for pre-designed AR scenes. Following that, we delve into the workflow of each of the system's main components. Finally, we detail the system's implementation specifics.

%\subsection{Background of AR Scene Structure}
%Our system is designed to process pre-crafted AR scenes as input. Thus, a brief overview of AR scene components is essential. There are various AR authoring systems exist, ranging from simpler ones like Reality Composer to more professional-facing platforms like Unity. To ensure our framework's versatility across most AR scenes, we use AR scenes created by Reality Composer as our input. This choice is due to its lightweight nature and its provision of essential information needed for our system's sound authoring. We employ this approach as a proof-of-concept. 

%While AR scenes from different tools might have slight structural or naming variations, they should be convertible to the similar format. Therefore, as long as other tools provide the required information, they can integrate with our framework.

%A standard AR scene comprises \textit{AR objects} and \textit{behaviors}. AR objects refer to 3D models, either static or animated, arranged in a user-defined layout. Every AR object possesses a filename that may indicate its nature or identity. If needed, a more detailed description can be embedded within the 3D model's metadata. Behaviors typically combine a trigger with an action. Triggers can be user interactions, such as tapping an AR object, the camera approaching an AR object, or a programmable event. In contrast, actions denote intended outcomes, like initiating an animation, causing an AR object to appear/disappear, or altering an AR object's position or orientation. In trigger-action-based AR authoring systems, users can associate triggers with actions, orchestrating the sequence of events in the AR scene. Many AR authoring tools, including Reality Composer, Adobe Aero, and Unity, offer trigger-action specification.

% Our system accepts pre-crafted AR scene as input. Thus, it is necessary to briefly introduce the basic components of an AR scene. 
% There exists many type of AR authoring system
% from some easy system like Reality Composer to more professional system like Unity. To make sure our system framework is generic enough to support most of the AR scene, we choose to use AR scene created by Reality Composer as input, as it is lightweight and contains the minimal set of information required for sound authoring by our system.
% We use this implementation as a proof-of-concept to illustrate our framework and other more complex tools be naturally adapted to the same framework. using the same framework as long as they have the necessary information required by our framework

\subsection{Event Textualization}
\label{subsection: event textulization}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/event_temp.png}
%     \caption{Event recognition.}
%     \label{fig:event}
% \end{figure}

In traditional AR authoring systems, creators manually specify which events can produce sound effects. These decisions are made during the authoring phase, with pre-determined sound effects provided by creator. As a result, users are limited to experiencing sounds associated with these specific events. Additionally, creators encounter several labor-intensive tasks in the authoring process: they must locate a matching sound source either by browsing or recording independently, identify all desired sound interactions and specify their triggers, and encode the contextual information for each AR interaction during authoring.

To simplify the creation of sound effects in AR and also incorporating context information into the sound authoring process, we introduce a Programming by Demonstration (PbD) authoring framework called SonifyAR. In our system, users first interact with the AR space before undertaking any authoring action. As user interactions take place, the system captures all AR events that can lead to sound feedback. Here we define an AR event as an user action and its subsequent result (\textit{e.g.} user tap a virtual object to trigger its animation). For each AR event, we describe it with an event type (\textit{e.g.} tapping an object or dragging a virtual item), action source (\textit{e.g.} user or virtual object), and action target (\textit{e.g.} virtual object or real-world plane). Information about the involved parties, such as virtual object or plane, will also be included in the context information \autoref{fig:pipeline}. This collected event data is then transformed into text, which is subsequently sent to the sound production component to craft the corresponding sound effect.

\paragraph{Event Types}
AR interaction contains a broad spectrum of action types. However, given our emphasis on sound authoring, we have narrowed our scope to focus on sound-related AR events. Specifically, we identify six types of events that could potentially trigger sound feedback. It is essential to note that these six events serve primarily as proof-of-concept. Users can easily adapt our methodology to accommodate any new event types not explicitly defined in our framework.
\begin{enumerate}
    \item Tap Real Word Structure: A user taps on a real-world structure through the AR interface.
    \item Slide: A user holds the virtual object and slide it on a real-world surface.
    \item Collide: A virtual object collides with a real-world surface. We implemented a specialized collision detection mechanism as introduced in \autoref{subsection:Implementation}
    \item Show Up: A virtual object show up in AR experience.
    \item Tap Virtual Objects: A user taps on virtual object through the AR interface.
    \item Play Animation: A virtual object plays an animation.
\end{enumerate}

\paragraph{Scene Context Understanding}
When the AR experience starts, SonifyAR utilizes ARKit \cite{apple-arkit-doc}'s plane detection functionality \cite{apple-arkit-plane-tracking} to understand the surrounding environment. Since most of the AR experiences are required to be anchored on planes, the detected plane information could serve as a crucial context information. To utilized such information, we employ the Deep Material Segmentation model \cite{upchurch_dense_2022} to segment the scene and identify the material of planes (\autoref{fig:pipeline} left). With the material segmentation results for each pixel of the camera stream, we could assign a material label to each detected planes. These material labels can help produce appropriate sound effects when either the AR object or the user interacts with real-world planes. Currently, we support six materials: Wooden, Carpet, Wall, Paper, Metal,and Glass. Surfaces that do not fall into one of these six categories are labeled as \textit{unknown surface}. %In the future, we can use a more advanced model to accommodate a broader range of materials.

\paragraph{Virtual Object Understanding}
In addition to real-world context, such as the planes and their material information, the semantics of the virtual object is also crucial for sound generation. To ensure sound assets align with the virtual object's material and its state, we collect a text description for all the virtual objects (\textit{e.g. "This model is a toy robot made of metal."}) and their animations (\textit{e.g. "A toy robot walks."}). These descriptions can be provided by the asset creator or, if necessary, we prompt the user to add relevant details. Any event involving the virtual object or its animation will incorporate these text descriptions.

\paragraph{Event-to-text}
As highlighted earlier, every event is identified and then translated into a text description which encapsulates the associated entities and actions. To structure these descriptions, we employ a simple text template. This template is designed as follows: \textit{"This event is [Event Type], caused by [Source]. This event casts on [Target Object]. [Additional Information on Involved Entities]".} Note that not all events have a target object or additional information, so these information can default. 

Breaking this down, here are the four core components of the template:

1) Source: The subject of the event, which could be the user when the event is directly triggered by user, or virtual object when it interacts with real-world environment.
2) Event Type: This is the type of event happened in AR interaction, described by the type name. 
3) Target Object: The object of the event, \textit{e.g.} the plane that gets tapped on, or the animation that gets played.
4) Additional Information on Involved Entities: Details that further elucidate the source object, the triggered event, and the target object. Examples encompass material descriptions of both the source and target objects and any animation details. %Users are asked to provide this data within the metadata of each 3D model.

During user interactions, the system actively monitors and logs the events happening in AR space. The relevant information about the Source Object, Triggered Behavior, and Target Object is fetched, including any supplementary details of the involved objects. All this data is then plugged into the text template, crafting a coherent description that reflects the user's interaction within the AR environment. 


% \paragraph{Pre-defined Event}
% As the AR scene begins to load, our system starts scanning the memory to identify which AR models have been loaded and what types of events have been designated for each AR object (e.g., appear/disappear, animation). Each event is then described as a natural language sentence using a template. \cmt{design and explain the template}. Once the template is populated with specific system components, the constructed sentence is sent to a language model to determine if the event requires sound. If a sound is necessary, we register this event in the "sound-producing event" list, and it is then queued for processing by the sound production component. Please refer to \cmt{Fig X} for an illustration.


% \paragraph{User Interaction Event}


\subsection{Sound Authoring}


\begin{figure}[h]
    
  \centering
  \includegraphics[width=0.7\linewidth]{Figures/SonifyAR Figure Generation.pdf}
  \caption{SonifyAR's sound acquisition pipeline. ``Method1'' is short for ``Method1recommend''.}
\label{fig:generation}
\end{figure}
%Need a figure here to explain the authoring pipieline, including the text content sent to and from the LLM.

In a traditional AR authoring system, users access a provided sound library to choose appropriate sound assets. If no suitable sound can be found in the library, users may search for sounds online or record sound by themselves. Once an ideal sound effect is identified, it can be added to the sound library and associated with a specific event. This sound authoring process can be labor-intensive and challenging, posing barrier to novice AR creators. With SonifyAR, we aim to simplify and automate this process using LLM and generative models to reduce the time and learning curve in AR sound authoring. 

SonifyAR utilizes the LLM to automatically find or generate context-matching sound assets of an AR event. Inspired by HuggingGPT\cite{shen2023hugginggpt} and Visual ChatGPT \cite{wu2023visual}, we utilize LLM as a controller of multiple sound authoring methods. LLM takes the text description of the event (described in \autoref{subsection: event textulization}) as input, and reply with commands for multiple sound authoring pipeline (\autoref{fig:generation}). In our current stage, we support three major sound authoring methods: recommendation, retrieval, and generation.

\subsubsection{Sound Recommendation} LLM can recommend sound assets based on semantics in the event description. Similar to other AR authoring tools, we collect a set of sound effects from Adobe Audition sound effects \cite{adobe-audition}, each labeled with a descriptive file name, like ``Crash Aluminum Tray Bang'' or ``Liquid Mud Suction''. The entire list of sound file name is provided to LLM as system context. When provided with text description of event, LLM selects the top five most suitable sound effects from the file name list, based on these self-explanatory file names. It then returns the selected sound effect in the format of \texttt{method1recommend:FILENAME}, where the \texttt{FILENAME} would be replaced with the actual filename. Upon receiving such command, SonifyAR would parse the filename and add the top corresponding sound as one of the sound options for event. An example reply from LLM regarding the recommendation process is shown in \autoref{fig:generation}, see "Recommend".

\subsubsection{Sound Retrieval} Since a finite collection of sound assets may not always contain the desired sound effect, we expand our sound authoring capability with online retrieval. We select the FreeSound \cite{freesound}, which is a non-profit online repository for sound, as the searching database. We utilize the FreeSound API, which returns a list of best matching sound effects from FreeSound based on a given query. We leverage the LLM to compress the entire event description into a shortened searching prompt (returned in the format of \texttt{method2retrieval:PROMPT}, where the \texttt{PROMPT} would be replaced with the search prompt), and search with such prompt using the FreeSound API. The returned results are JSON strings including information of all search results. We then let LLM select the top five matches from the entire set of sound effects returned by the API, by comparing the text descriptions of the returned sound effects with our input text description. The top one result will be downloaded and presented to user as one of the sound options. Others in the top five alternatives are also stored in our system for users who wish to explore more options. This retrieval process is shown in the bottom right of \autoref{fig:generation}.

\subsubsection{Sound Generation} Since our system already operates with text descriptions as input, we naturally adopt text-to-audio generation model (AudioLDM~\cite{liu2023audioldm} in our implementation) as an intuitive choice for generating sound effects to complement the previous approaches. We ask the LLM to compress the event text description into a shortened generation prompt (returned in the format of \texttt{method3generation:PROMPT}, where the \texttt{PROMPT} would be replaced with the generation prompt). Upon receiving such command from LLM, SonifyAR will send the prompt to the AudioLDM model, requesting text-to-sound generation. This newly generated sound are then stored in our system for user exploration at a later time. 

Additionally, the audio diffusion model can also conduct text-based style transfer and generate similar sound functionality, which we also utilize in SonifyAR system. Specifically, when generating sound effects for tapping, sliding or colliding events, we will pass a default sound effect and request a style transfer operation with text prompt (see ``Generate'' in \autoref{fig:generation}), instead of generating a new sound from scratch. This pipeline could let the output sound has similar length and rhythm of the input sound, ensuring a good time match of sound with events. Also, when user want to modify a certain sound in the provided options, SonifyAR also offer text-based style transfer or generating similar sound as possible operations, enabling user to iterate and edit the sound assets.

All sound authoring process listed above, including recommendation, generation and retrieval processes, simultaneously run in parallel on the backend, ensuring no interference with the user's AR experience. 



% We use three types of technique to generate sound given a text description.
% 1. retrieve on collection (LLM recommendation based on title)
% 2. retrieve on online resources (we use freesound)
% 3. text-to-sound generation (AudioLDM), explain details in implementation (if else).

\subsection{User Interface}

%Need an interface figure
\begin{figure}[h]
    
  \centering
  \includegraphics[width=0.7\linewidth]{Figures/SonifyAR Figure Interface.pdf}
  \caption{SonifyAR's authoring interface. Left: SonifyAR's phone-based AR interface. Right: SonifyAR's authoring panel.}
\label{fig:interface}
\end{figure}
Our system adopts a PbD authoring framework that enables users to author sound effects interactively while engaging with the AR environment. This approach offers a more intuitive authoring experience by helping users understand the relationship between their interaction behaviors and the potential generated sound effects.

To support this experience, our system blurs the line between the authoring and demonstration stages. We initiate our system directly with an interactive AR experience (\autoref{fig:interface} left). Users can freely interact with the scene, performing actions like moving virtual objects or interacting with the real-world surfaces. When an AR event is detected, a text label appears on the top-left screen to inform the user (\autoref{fig:interface}.A), and the sound acquisition component is activated to generate candidate sound effects for the detected events.

By clicking a button (\autoref{fig:interface}.D), users can prompt an editing interface that overlays on the AR scene. The interface includes all unique AR events detected (\autoref{fig:interface}.H) and the automatically generated sound effects (\autoref{fig:interface}.I), enabling users to explore the detected events and their corresponding sound effects.. Users can click on a sound effect to preview it and double click to select and activate it during the AR session if it is suitable. After confirming their choices, users can minimize the authoring panel (\autoref{fig:interface}.G) to resume the AR experiences and test the selected sound. Users can always access the editing interface to modify their choices if necessary.

Furthermore, users can long press a sound asset to call out a menu with a suite of exploratory options. For recommended or retrieved sound, the menu would include an option to list all other sound assets in the top five recommendations. For all sound assets, the menu provides a ``style transfer'' and a ``generate similar sound'' features, enabling users to transfer audio effects or to generate a new similar sound based on the selected sound. When this feature is selected, users can type a simple text prompt to guide the sound generation process. This feature lets users iteratively refine sound effects and explore new sound variations.



\subsection{Implementation}
\label{subsection:Implementation}
To enable the interaction and sound generation pipeline of SonifyAR, we developed a mobile app with user interface that enables AR interaction and sound authoring actions. We also implemented back-end servers for scene understanding and sound generation. The current SonifyAR demo is built with Apple's ARKit with Swift 5.7 and Xcode 14, and runs as an iOS application on iPhone. Due to the enhanced performance of plane detection on devices with LiDAR (available in iPhone's Pro lineup starting from iPhone Pro 12), we developed and tested the app on an iPhone 13 Pro Max running iOS 16. We implemented the collision detection between virtual objects and planes with ARKit's physics simulation \cite{apple-scenekit-physics-simulation} function. To enable collision detection for animated virtual object parts (\textit{e.g.} the stomping of robot foot on plane), we bind collider to the joints of the virtual object's animated bones.

We use GPT-3.5 as the LLM API used in our system considering its superior performance and quick response time. We adopt the DMS model 
\cite{upchurch_dense_2022} for material segmentation because of its detailed material labeling, fast processing time, and high accuracy. The model is hosted remotely with an Nvidia RTX 2060 GPU and CUDA 10.1. The deployed model communicates with the iOS app via Flask. For sound generation, we use the AudioLDM model \cite{liu2023audioldm} due to its state-of-the-art performance and its flexibility regarding text input and operation types. This model is hosted on a server with Tesla T4 GPU with Cuda 12.2.



% Implementation details on what exact model/algorithm used for each component, and our device used for testing.

% We want to emphasize that our system is focusing on sound authoring, so we need to take authored AR scene as input because creating AR scene is beyond the scope of our system. This makes our system to be use as an add-on to any other AR authoring tools like Aero. Once the AR scene is authored and launched, we initiate our system to generate sound effect to the scene.



% Some overview of the pipeline, with the diagram.
% \subsection{Context as text}
% Collect context information from multiple sources and models, turn them into text.
% \subsection{Sound from context}
% With the text containing context information, we could generate/retrieve/transfer sound to adapt to context.

% We use sound generation model, sound retrieval API, and recommendation of LLM.
% \subsection{User interaction}
% We consider user intention as part of the context information. Thus engaging user in a interaction pipeline is necessary. user could express their design intention and preferences over multiple choices in an iterative interaction based on language and UI taps.

==> Sections/Archive/6-Evaluation.tex <==
\section{Evaluation}
To examine the usability and authoring performance of the SonifyAR system, we conducted two studies across a total of 13 participants. The first study is a usability study that include user's operation of the SonifyAR application, aiming to measure its usability and technical performance. Participants provided ratings for several questions about the system, and also elaborated on their general feedback and reasonings behind ratings. The second study is an interview with five AR experts focusing on the interaction design of the SonifyAR system. We let the participants compare our system with commercial AR authoring tool and collected their feedback as well as their opinions on potential application scenarios of our system.

\subsection{Study One: Usability Study}
\subsubsection{Participants}
The first study involves eight participants with varying experience in AR. The eight participants (6 male and 2 female) age between 26 and 33. We inquired about their prior experience in AR before the study. Out of the eight participants, six had prior AR experience, and three had experience in AR authoring tools.

\subsubsection{Procedure}
The usability study was conducted in an office setting and comprised four steps. We first introduce our study goal with the participants and collect answers to our demographic questions. We then demonstrated our SonifyAR app with a sample AR experiences. During this phase, participants had the opportunity to clarify any uncertainties regarding SonifyAR's functionalities to ensure a comprehensive understanding of the tool's capabilities. Afterwards, participants were given the chance to independently explore the SonifyAR app. We provided a walking robot model which can be added to indoor surfaces. This model starts walking when tapped. We asked the participants to explore this AR asset freely and use our automatic sound authoring pipeline to create sound effects with the model until they found the results satisfactory. The entire usage process was screen-recorded and the user operations were logged. The final step involved asking questions regarding the usability, helpfulness and technical performance of the SonifyAR system based their personal experiences. Participants also provided reasoning and insights to support their answers. The questions and rating results are shown in \autoref{fig:stats}.

\subsubsection{Usability Study Results}
All participants were able to complete the AR sound authoring task using SonifyAR without difficulty. On average, the authoring process took 406 seconds (SD=137s) to finish. Participants tested on an average of 56 (SD=10.48) sound assets, with 6.4 sounds (SD=1.67) gets assigned to the authoring results.

Feedback on the SonifyAR app was largely positive. All eight participants expressed a favorable impression of the tool. They were highly agreed that the SonifyAR tool would be helpful to AR authoring process (Q1,AVG=6, SD=0.93). There was also a general willingness for using SonifyAR in their own AR creation practice (Q2, AVG=6.25, SD=1.16). Participants agreed that the sound interaction involving the real world surfaces will improve the immersiveness of AR experiences (Q3, AVG=6.38, SD=1.06). Additionally, they preferred the automated sound authoring process over the manual search for sound assets (Q5, AVG=6.13, SD=0.99). The only area for improvement was the quality of the generated sound (Q4, AVG=4.75, SD=1.39). However, this could be enhanced with the introduction of a more advanced sound generative model, which we could readily integrate into our system. The full Likert-type results can be viewed in \autoref{fig:stats}.

\begin{figure}[h]
    
  \centering
  \includegraphics[width=0.75\linewidth]{Figures/SonifyAR Stats.pdf}
  \caption{Likert-type questions and results of usability study}
\label{fig:stats}
\end{figure}

\subsection{Study Two: Expert Interview}
\label{subsec:expert interview}
\subsubsection{Participants}
To further gather feedback and evaluate our contribution to the AR authoring process, we recruited five AR experts from both research institutes and software development industry. These five experts (4 female and 1 male, aged between 25 to 34) all have extensive experiences with both AR and AR authoring tools.

\subsubsection{Study Procedures}
The interview consisted of three steps. First, we introduced the goal of our study and collected responses to demographic questions, which were same as those in study one. Next, we provided a live demonstration of Adobe Aero and SonifyAR to enable a comparison of these two AR authoring tools and the PbS and PbD authoring methodology they represent. Lastly, we asked several questions about the authoring process of these two applications, seeking insights on their key differences and general preferences among our five AR experts. The interviews were recorded and transcribed for analysis. Below, we present the three questions asked during the interview and their respective responses.

\paragraph{Question One: What are the pros and cons of each AR authoring method?}
In traditional PbS or trigger-action-based system, a common drawback reported is their tendency to be laborious and demanding in terms of skills and design thinking. Nevertheless, these higher skill requirements and workload also confer greater flexibility and control over the authoring process. As one expert aptly put it, \textit{``I would say PbS authoring is definitely more tedious but also gives you more flexibility in doing different things ... but I guess if you do have the idea, it might be faster (than PbD authoring).''}

Conversely, for the PbD authoring process in SonifyAR, experts perceived several advantages. It is considered beneficial for exploring the design space and features a gentle learning curve, making it more accessible for novice users. Furthermore, with the integration of generative models, SonifyAR becomes a valuable tool for brainstorming and iterative design. However, experts expressed concerns that PbD authoring might lack the depth or granularity of authoring compared to PbS methods.

Two experts advocated for merging the strengths of both methods in the AR authoring pipeline. They suggested utilizing PbS authoring for structured and detailed design, while SonifyAR assists in generating sound assets and proposing sound-related events during testing, thus expediting and enriching the design iteration.
%For the traditional PbS methods, a common disadvantage reported is being tedious to use and requires more skills and overall design thinking. But this higher requirement of skills and workload also brings more flexibility and control over the authoring process. One said: "I would say [the PbS authoring] is definitely more tedious but also gives you more flexibility in doing different things ... but I guess if you do have the idea, it might be faster [than the PbD authoring]."

%For the PbD authoring, experts believe that it's beneficial for exploring the design space and have shallow learning curve, thus better for novice users. It's also beneficial to brainstorming and iteration of design thanks to the application of generative models. However, the PbD authoring also limits the granularity of authoring. 

\paragraph{Question Two: How would you describe your preferences between these two authoring methods?}
One expert showed clear preference over the SonifyAR authoring process over the PbD methods. The other four experts expressed a balanced preferences over these two methods, noting that each has its advantages and disadvantages and is suited for different scenarios.. One expert remarked, \textit{``I guess it depends on what kind of a designer I am or the purpose of the task. If I'm a sound design engineer, then I might want full control (thus prefer PbS authoring). But for someone who doesn't have an expertise in that realm, but would still like to make my AR experiences more immersive, I probably want the generative thing because I just need some suggestions.''}
\paragraph{Question Three: Do you have any potential concerns regarding the PbD authoring method showcased in our SonifyAR tool?}
Experts voiced concerns about some missing fuctionalities over sound editing, like trimming and adjusting volumn and pitch. Besides these implementation level deficits, one notable concern is the PbD authoring process might struggle when faced with managing numerous events simultaneously, potentially overwhelming the user interface. Another concern is that the dependence on the generative models might be inadequate for scenarios not yet robustly addressed by current models. This could, in turn, limit users by confining them to the outcomes generated by the models.

%\subsubsection{Findings}
%Besides the ratings we received, we also solicited qualitative feedback from participants. We summarize these findings into three main insights:
%\subsubsection{Usability of tool}
%Participants were pretty satisfeid with the overall usability of the tool. However, there can be some UI level improvements that could potentially improve user experiences.

%\subsubsection{Generation Results}
%Pretty good in general, good enough to express textual difference and event semantics. Could be improved if better models come out in the future or we train or fine tune model by ourselves.

%\subsubsection{Comparison between PbD and PbS authoring}
%Event-based more useful for amateur users. Trigger-action more useful for pros. But probably we could combine them together since they are useful in different phases of authoring.


%\subsubsection{Study One: Hands on of SonifyAR}
%Study one is conducted in person in an office room and includes three steps. We first introduce our study goal with the participants, collect answers to our demographic questions, and showed our SonifyAR demo application by hands-on demonstration. Then participants get to try out the SonifyAR application independently. We provided a given virtual model and let them freely author sound effects with the model until satisfactory. The entire usage process is screen recorded. The final step is asking several questions for their ratings of the general experiences and their evaluation of the system's technical performance. Participants also provided reasoning and insights for their answers.
%\subsubsection{Study Two: Comparison of SonifyAR with Adobe Aero}
%Study two is conducted remotely over Microsoft Teams and include three steps. We first introduce the goal of our study and collected answers to our demographic questions, which are same as study one. We then live showcased Adobe Aero \cite{adobeaero} and SonifyAR with screen sharing on phone. Lastly, we ask several questions about the authoring process of these two applications, and solicit insights of key differences and general preferences among our five AR experts.

%Questions asked in study one and study two are listed in \autoref{tab:questions}

% add the table here.
%\input{Tables/Questions}

%\subsection{Data Analysis}
%For both studies, we recorded most of the interview process, except for one in-person participant who preferred not to be recorded. We transcribed all the interview recording and extracted common feedback and insights. For the only non-recorded study, we took down all key answers during the interview. The study results, including numerical ratings for the system and qualitative feedback, are shown below in \autoref{tab:results}. Besides collecting answers to questions, we also analyzed the screen recording of users' hands-on of the SonifyAR application for some stats in their usage habits.

%\input{Tables/Results}
%\subsection{Study Results}
%Overall, all in-person participants could easily finish AR sound authoring with SonifyAR. The average authoring process takes ?? to finish, and an average of ?? sound assets gets tried out, with ?? get assigned. Participants are generally satisfied with the SonifyAR demo application, with all eight in-person participants indicating positive overall impression of the tool. Participants are also generally positive about the helpfulness (Q2, with average rating 6 out of 7) and immersiveness (Q4, with average rating of 6.43 out of 7). Participants also expressed that they would like to use the tool in their own practice (Q3, with average rating of 6.17 out of 7), and preferred the automated sound authoring process over the manual search for sound assets (Q6, with average rating of 6.13 out of 7). The only weakness in evaluation is the quality of the generated sound (Q5, with average rating of 4.75 out of 7).



==> Sections/Archive/7-Discussion.tex <==
\section{Discussion and Future Work}
In this paper, we designed and implemented an AR sound authoring pipeline that automatically generates sound assets based on context information. We evaluated and discovered the opportunities in the AR sound interaction space, and implemented a LLM+Generative AI pipeline for sound acquisition. We tested the pipeline with a usability study on an iOS demo application and further discussed the overall contribution and application opportunity with an interview with AR experts.

%\subsection{Sound quality}
%Based on our usability study results (\autoref{}), participants are generally satisfied with the system's usability and technical performance. However, according to multiple comments, the quality of the acquired sound can still be improved, especially for the text-to-audio generated sounds.
%We argue that although the current sound generation quality is not perfect, the text-to-audio generation is a new and popular research field with countless emerging work. And with natural language as the input modality, we can always replace the current AudioLDM model with better future models. In this case, the SonifyAR system leaves open ports for future iterations and improvements.

\subsection{Usage Scenarios}
%As discussed in the expert interview (\autoref{}), the SonifyAR system can be useful in many application scenarios. 
\paragraph{E-commerce}
AR is widely adopted as presentation medium in e-commerce sites like Amazon and IKEA. We envision SonifyAR could further strengthen the e-commerce AR experiences by adding material-aware sounds. For example, SonifyAR can help make a virtual ceramic cup chime when being touched or moved. These sound feedback can improve the media novelty and immersion of the AR experience, which according to prior experiment \cite{yim2017augmented} boost people's purchase intention.
\paragraph{Accessibility}
Existing research ~\cite{zhao2019designing,zhao2020effectiveness,ribeiro_auditory_2012} explored assisting blind or low vision (BLV) people with AR in two modalities: visual highlights and audio hints. SonifyAR is in alignment with the latter approach by simplifying the sound authoring process.  Additionally, SonifyAR enables new AR sound interaction-the user-reality sound interaction (see \autoref{section:design space})-that can help BLV people explore the real world space through AR interfaces.
\paragraph{Plug-in to existing platforms}
In our expert interview (see \autoref{subsec:expert interview}), several AR specialists proposed that SonifyAR could seamlessly integrate into established AR authoring tools. Given that the authoring pipeline of existing tools precedes the AR experiences, while our PbD (Programming by Demonstration) pipeline operates concurrently during these experiences, these two methods occupy distinct time segments and, as such, can complement each other effectively.

Traditionally, creators followed an author-test-author iteration process when crafting AR experiences. With the introduction of SonifyAR, which identifies authorable events and generates corresponding sounds during the testing phase, this iterative authoring process gains significant acceleration. Furthermore, it simplifies the specification of intricate sound interactions and draws attention to often overlooked sound-related aspects.

%In our expert interview (\autoref{}), multiple AR experts suggest that SonifyAR can be incorporated into existing AR authoring tools. Since the authoring pipeline of the existing tools happens before the AR experiences and our PbD pipeline happens during the AR experiences, these two methods are segmented in time thus can be complementary to each other. Traditionally, creators would author AR experiences in a author-test-author iteration. With SonifyAR pointing out authorable events and generating sound in the test phase, it accelerates the iterative authoring process, simplifies the specification of complex sound interactions, and hints on the easily neglected sound interactions.
\subsection{Future work}
%In the future, we plan to continue improving the SonifyAR pipeline in terms of UI/UX, technical performance, and seek applicatiopn within existing AR authoring frameworks.
%Improve UI/UX.
%As suggested by the user evaluation, our PbD authoring process can provide better visual hints to link the sound interaction with sound asset options.
While SonifyAR enables automated AR sound authoring, there remains room for further opportunities and enhancements.

Firstly, our current SonifyAR app is a simplified tool compared to comprehensive AR design suites that cover every aspect of AR scene creation. It exclusively supports the authoring of AR sound and accepts pre-crafted AR scenes as input. For wider applicability that reflects the real-world intricacies of AR content creation, we recognize the need to extend its capabilities to accommodate a wider spectrum of AR events and interactions.  Our future goals include integrating the SonifyAR framework with established tools like Reality Composer and Adobe Aero.

Secondly, SonifyAR adopts a straightforward process of collecting context information for virtual objects by using a text template to compile semantics. In future developments, we aspire to incorporate computer vision models for object detection and image understanding,  thus enhancing the context acquisition process with greater precision and broader adaptability.

Lastly, the current sound generation output of SonifyAR presents opportunities for further refinement. Recognizing the rapid advancements in the AI research domain, our system has been designed as a modular framework, ensuring that as more advanced models emerge, they can be seamlessly integrated. Every LLM/CV/generative model within SonifyAR is replaceable, allowing SonifyAR to easily adapt and stay at the forefront of innovation in this field.

==> Tables/Questions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Questions asked in two studies}
  \label{tab:questions}
\begin{tabular}{l|lc}
\hline
                                                                                                       & \multicolumn{1}{c|}{\textbf{Study One}}                                                                                                                                                                                                                                         & \textbf{Study Two}                                                                                                      \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Demographic\\  questions\end{tabular}}} & \multicolumn{2}{c}{Age}                                                                                                                                                                                                                                                                                                                                                                                   \\ \cline{2-3} 
\multicolumn{1}{c|}{}                                                                                  & \multicolumn{2}{c}{Experience in AR (1 no experience - 7 very experienced)}                                                                                                                                                                                                                                                                                                                               \\ \cline{2-3} 
\multicolumn{1}{c|}{}                                                                                  & \multicolumn{2}{c}{Experience in AR authoring tools (1 no experience - 7 very experienced)}                                                                                                                                                                                                                                                                                                               \\ \hline
Q1                                                                                                     & \multicolumn{1}{l|}{How do you like this demo application in general?}                                                                                                                                                                                                          & \begin{tabular}[c]{@{}c@{}}How would you describe your preferences\\  between these two authoring methods?\end{tabular} \\ \hline
Q2                                                                                                     & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Do you think this authoring process is helpful?\\  (1 very unhelpful-7 very helpful)\end{tabular}}                                                                                                                               & What’s the pros and cons of each method?                                                                                \\ \hline
Q3                                                                                                     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Do you think you will use this authoring process if you are doing AR content creation? \\ (1 definitely no - 7 definitely yes)\end{tabular}}                                                                                                                                                                                                                \\ \hline
Q4                                                                                                     & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Do you think the user-environment interaction will\\  increase the immersiveness of AR experience? \\ (1 not at all – 7 increase a lot)\end{tabular}}                                                                            & \begin{tabular}[c]{@{}c@{}}Do you have any other concerns \\ about the PbD authoring method?\end{tabular}               \\ \hline
Q5                                                                                                     & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}How do you like the sound authoring results? \\ (1 not at all – 7 Like it very much)\end{tabular}}                                                                                                                               & \multicolumn{1}{l}{}                                                                                                    \\ \cline{1-2}
Q6                                                                                                     & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}How do you like the automatic sound generation \\ process? Compared to recording/searching a sound\\  by yourself, which one do you prefer? (1 I would \\ like to search or record– 7 I like to use generative AI)\end{tabular}} & \multicolumn{1}{l}{}                                                                                                    \\ \cline{1-2}
Q7                                                                                                     & \multicolumn{1}{l|}{Do you have any other comments or suggestions?}                                                                                                                                                                                                             & \multicolumn{1}{l}{}                                                                                                    \\ \hline
\end{tabular}
\end{table}

==> Tables/Results.tex <==
\begin{table}[]
\caption{Study results. Numbers are based on 1-7 ratings for each question. Exp is short for experience. AT is short for authoring tools. The missing girds are not asked or not answered by participant.}
  \label{tab:results}
\begin{tabular}{llccc|ccccc}
\hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Participant \\ No.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}In person\\ or remote\end{tabular} & \multicolumn{1}{l}{Age} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Exp \\ in AR\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Exp in \\ AR AT\end{tabular}} & \multicolumn{1}{l}{Q2}   & \multicolumn{1}{l}{Q3}   & \multicolumn{1}{l}{Q4}   & \multicolumn{1}{l}{Q5}   & \multicolumn{1}{l}{Q6}   \\ \hline
\multicolumn{1}{l|}{P1}                                                         & In person                                                     & 26                      & 3                                                                        & 1                                                                            & 6                        & 7                        & 7                        & 6                        & 5                        \\
\multicolumn{1}{l|}{P2}                                                         & In person                                                     & 26                      & 4                                                                        & 5                                                                            & 5                        & 5                        &                          & 3                        & 6                        \\
\multicolumn{1}{l|}{P3}                                                         & In person                                                     & 33                      & 1                                                                        & 1                                                                            & 7                        & 7                        & 7                        & 6                        & 7                        \\
\multicolumn{1}{l|}{P4}                                                         & In person                                                     & 31                      & 4                                                                        & 3                                                                            & 5                        & 4                        & 4                        & 3                        & 5                        \\
\multicolumn{1}{l|}{P5}                                                         & In person                                                     & 27                      & 3                                                                        & 1                                                                            & 7                        & 7                        & 6                        & 6                        & 7                        \\
\multicolumn{1}{l|}{P6}                                                         & In person                                                     & 32                      & 3                                                                        & 1                                                                            & 7                        & 6                        & 7                        & 6                        & 7                        \\
\multicolumn{1}{l|}{P7}                                                         & In person                                                     & 26                      & 1                                                                        & 1                                                                            & 5                        & 7                        & 7                        & 4                        & 7                        \\
\multicolumn{1}{l|}{P8}                                                         & In person                                                     & 29                      & 4                                                                        & 3                                                                            & 6                        & 7                        & 7                        & 4                        & 5                        \\ \hline
\multicolumn{1}{l|}{P9}                                                         & Remote                                                        & 26                      & 6                                                                        & 5                                                                            &                          & 4                        &                          &                          &                          \\
\multicolumn{1}{l|}{P10}                                                        & Remote                                                        & 25                      & 5                                                                        & 5                                                                            &                          & 7                        &                          &                          &                          \\
\multicolumn{1}{l|}{P11}                                                        & Remote                                                        & 26                      & 7                                                                        & 7                                                                            &                          & 7                        &                          &                          &                          \\
\multicolumn{1}{l|}{P12}                                                        & Remote                                                        & 25                      & 5                                                                        & 7                                                                            &                          & 6                        &                          &                          &                          \\
\multicolumn{1}{l|}{P13}                                                        & Remote                                                        & 34                      & 7                                                                        & 7                                                                            &                          &                          &                          &                          &                          \\ \hline
\multicolumn{5}{r|}{Average}                                                                                                                                                                                                                                                                                                        & \multicolumn{1}{r}{6.00} & \multicolumn{1}{r}{6.17} & \multicolumn{1}{r}{6.43} & \multicolumn{1}{r}{4.75} & \multicolumn{1}{r}{6.13} \\ \hline
\end{tabular}
\end{table}
